Promises and Challenges of Causality for Ethical Machine Learning

In recent years, there has been increasing interest in causal reasoning for designing fair decision-making systems due to its compatibility with legal frameworks, interpretability for human stakeholders, and robustness to spurious correlations inherent in observational data, among other factors. The recent attention to causal fairness, however, has been accompanied with great skepticism due to practical and epistemological challenges with applying current causal fairness approaches in the literature. Motivated by the long-standing empirical work on causality in econometrics, social sciences, and biomedical sciences, in this paper we lay out the conditions for appropriate application of causal fairness under the "potential outcomes framework." We highlight key aspects of causal inference that are often ignored in the causal fairness literature. In particular, we discuss the importance of specifying the nature and timing of interventions on social categories such as race or gender. Precisely, instead of postulating an intervention on immutable attributes, we propose a shift in focus to their perceptions and discuss the implications for fairness evaluation. We argue that such conceptualization of the intervention is key in evaluating the validity of causal assumptions and conducting sound causal analysis including avoiding post-treatment bias. Subsequently, we illustrate how causality can address the limitations of existing fairness metrics, including those that depend upon statistical correlations. Specifically, we introduce causal variants of common statistical notions of fairness, and we make a novel observation that under the causal framework there is no fundamental disagreement between different notions of fairness. Finally, we conduct extensive experiments where we demonstrate our approach for evaluating and mitigating unfairness, specially when post-treatment variables are present.

==> experiments_FAccT.tex <==
\section{Empirical Results}\label{sec:experiments}
%We illustrate the fairness evaluation and mitigation using synthetic and real-world datasets. 
%simulate a hiring scenario, where we investigate the different stages that discrimination can creep into the decision-making process and we study how the choice of timing impact our conclusions. We conclude by a case study using the Home Mortgage Disclosure Act dataset (HMDA), where we demonstrate our approach for mitigating unfairness. 
We consider a stylized hiring scenario to illustrate our causal unfairness evaluation and mitigation approach. Specifically, we consider a decision-making process that involves two interactions: interview and final hiring decision. We study how the timing of the intervention impacts our conclusions.
%We synthesize data so that we can compare fairness definitions in a setting where we observe the potential outcomes. 
We use $A$ to represent gender, which we draw from a Bernoulli distribution $\textit{Bern}(0.75)$ with the majority class being male $A=1$. An individual's qualification is described by a random variable $X$ drawn from a normal distribution $\mathcal{N}(2\alpha(A - 0.5), 1)$, where $\alpha$ controls the difference in the average qualifications between genders. Each candidate has a score $S$ reflecting their performance during the interview. We model the score as a binary variable whose mean depends on the qualifications and possibly gender. We have $\mathbb P(S = 1) = \sigma\left(X + 2\beta (A - 0.5)\right), $ where $\sigma(z) = 1/(1+e^{-z})$ is the logistic function and $\beta \geq 0$ determines the level of discrimination in $S$, e.g., when $\beta > 0$ being a male $A = 1$ increases one's probability of receiving a higher score. Subsequently, a decision $Y$ is made indicating whether the candidate receives an offer or not. We use the probabilistic model $\mathbb{P}(Y = 1) = \sigma\left(X + S +  2\gamma(A - 0.5)\right)$, with $\gamma \geq 0$ controlling the level of discrimination in $Y$ for a fixed $X, S$. The vector of potential outcomes, for both $S$ and $Y$, can be obtained by substituting the respective value of $A$ in the model. 
We present results across a wide range of $\alpha, \beta$ and $\gamma$ values. 
%For post-interview fairness evaluation we can use the observed $S$ values as the score is a pre-treatment variable (See Equation~\ref{eq:pre-treatment-evaluation}).

%\in \{0, 0.1, 0.5, 1, 1.5, 2\}, \gamma \in \{0, 0.12, 0.14, 0.16, 0.18, 0.20\}.$ 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/causalVSstatistical_beta.pdf}
    \caption{Synthetic results in the hiring scenario. Colors denote the evaluation method: causal pre-interview, causal post-interview and statistical. From top to bottom, each row corresponds to a different value of $\alpha \in \{-0.5, 0, 0.5\}$. Column are different fairness evaluation criteria. On the $x-$axis, we vary the value of $\beta$, which reflects the dependence of the interview score on one's gender. The $y-$axis shows fairness violation across four different definitions.
    We note that for causal approaches we use the causal variants of the fairness definitions.
    The value of $\gamma$ is set to 0.2. The error bars show 95\% confidence interval. Depending on the joint setting of the parameters, statistical criteria may erroneously result in an over- or under-estimation of fairness violation. Further, post-interview fairness evaluation does not capture discrimination at earlier points in time.}
    \label{fig:synthetic}
    \vspace*{-\baselineskip}
\end{figure}

According to our causal framework, we need to specify the point in time from which the effect of gender needs to be assessed. There are two possibilities: after interview is conducted or before the interview (as one may be concerned about an unfair interview process). Naturally, the above choice will impact our conclusions about whether the system is fair or not. We generate 100,000 data points $(X, A, S(0), S(1), Y(0, S(0)), Y(1, S(1)))$ according to the process explained above. For post-interview fairness evaluation we can use the observed $S$ values as the score is a pre-treatment variable. However, when evaluating fairness before the interview, the score becomes post-treatment. In order to impute the missing counterfactual score values $S(A)$, we use logistic regression to model $\P(S = 1 \mid \bm X = \bm x, A = a), \; a \in \{0, 1\},$ from which we sample (10 samples). We use a second logistic regression $\P(Y = 1 \mid \bm X = \bm x, S(a) = s, A = a), \; \forall a,s \in \{0, 1\}$ to impute $Y(A, S(A))$ values. This approach is based on multiple imputation in the causal inference literature~\cite{Rubin1996MultipleYears}. We then use these counterfactual values in the expression that evaluates the treatment effect of $A$. 



We compare our causal criteria against statistical fairness definitions, where we measure the fairness violation of a logistic regression model trained to predict $Y$ using observed values of $X, S$ and $A$. Figure~\ref{fig:synthetic} depicts a summary of results. 
%On the $x-$axis, we vary the value of $\beta$, which reflects the dependence of the interview score on one's gender. The $y-$axis shows fairness violation across four different definitions. The results are replicated for three different values of $\alpha = \{-0.5, 0, 0.5\}$ shown on the right-hand side of the figure. The value of $\gamma$ is set to $0.2$.


We can make several key observations. First, the post-interview causal plot remains flat across different values of $\alpha, \beta$ exhibiting a constant fairness violation at 0.07 due to constant $\gamma = 0.2$ which is independent of prior discrimination in the interview step. This suggests that early discrimination can not be captured when one chooses a later time as the point of fairness investigation. In other words, any unfairness in the pre-treatment variables used in the analysis will remain undetected. Pre- and post-interview lines only intersect at $\beta = 0$ and pre-interview fairness violation increases monotonically with $\beta$ across all causal fairness definitions. 
%, even though causal equalized odds (TP) and (FP) show less sensitivity to variations in $\beta$\newar{Why?}.
Statistical fairness definitions exhibit significantly different results. For example, when $\alpha = -0.5$, all statistical lines lie below the causal ones which suggests that they underestimate the true level of discrimination. This is due to the fact that when $\alpha < 0$, males qualification is lower than females on average. However, since $\beta, \gamma > 0$ the interview score and the final decision are in favor of male candidates. Since the statistical criteria fail to disentangle different sources of disparities, these opposing effects are cancelled, resulting in lower estimates of unfairness. On the other hand, when $\alpha > 0$, these effects reinforce each other resulting in an over-estimation of unfairness. Only when $\alpha = 0$, do statistical parity and causal parity, in Causal (Pre), match which indicates the sensitive of statistical criteria to baseline differences between groups (average qualifications). 
For $\beta, \gamma = 0$ (no discrimination in interview or the hiring process), our results indicate near-zero estimates for all causal definitions of fairness across different values of $\alpha$. This confirms that it is indeed possible to satisfy  different causal fairness definitions simultaneously, even when there are baseline differences between the qualifications of different groups. Conversely, statistical criteria yield non-zero estimates except for the case where $\alpha, \beta, \gamma = 0$ which points to the equal base rate condition highlighted in previous work~\cite{Kleinberg2017InherentScores}. 
% \begin{figure}[t]
%     \begin{subfigure}[b]{\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/causalBeforeInterview.pdf}\caption{Fairness considered before the interview}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/causalAfterInterview.pdf}\caption{Fairness considered after the interview}
%     \end{subfigure}
% \end{figure}


%When interview is unfair, the subsequent decision is arguably unfair, however, as we show

%\noindent\textbf{Criminal Justice System. }We use COMPAS dataset used in~\cite{angwin2016machine}. Judges are often presented with two sets of scores from the COMPAS system -- one that classifies people into High, Medium and Low risk, and a corresponding decile score --> under strong assumptions, we can use this dataset to learn whether the judges have been discriminatory (does it have actions). Clearly, a fair judge if provided misinformation or information that doesn't truly reflect one's risk of re-offense can lead to unfair decisions. So the input to these models should be accurate, for each group, to begin with. However, the COMPAS data does not provide this level of granularity. The judges decision is not available in the data. Can we impute this column semi-synthetically? 
Next, we study the power of our approach to mitigate unfairness. We focus on the setting where $\alpha = 0$ and $\beta, \gamma \neq 0$. This is because we aim to remove unfairness in the decision-making process, which is associated with $\beta$ and $\gamma$. Since statistical approaches are not able to disentangle different sources of unfairness, by setting $\alpha$ we are able to compare our results against those criteria. Specifically, we train a model using our approach by imputing the missing potential outcomes. We compare the accuracy and fairness violation with an unconstrained model (No Fairness), as well as the
same model after applying one of three common unfairness mitigation algorithms in the literature: pre-processing method (Re-weighting) in~\cite{Kamiran2012DataDiscrimination} which generates weights for the training examples in each combination of $A$ and $Y$ differently to ensure statistical parity, in-processing method (PrejudiceRemover) of~\cite{Kamishima2012Fairness-awareRegularizer} that adds a regularization term to the learning objective, and post-processing approach (RejectOption) in~\cite{Kamiran2012DecisionClassification} which gives favorable outcomes to unprivileged groups and unfavorable outcomes to privileged groups in a confidence band around the decision boundary. We rely on the implementations in AI Fairness 360 package~\cite{Bellamy2018AiBias}. The training model used in all of the methods is a logistic regression model. For fairness violation, we consider both statistical criteria and their causal variants.

Table~\ref{tab:res-total-stat} summarizes the statistical fairness violation results for $\beta = 1.0 $ and $\gamma = 0.2$. Among all fair baselines, RejectOption and Causal (Pre) perform significantly better in terms of statistical parity. Despite the fact that other fair baselines are also designed to remove average disparities between groups, they still exhibit significant disparities. On the other hand, RejectOption performs worse than Causal (Pre) with respect to all other criteria. 
%Causal (Pre) outperforms re-weighting method in parity. 
%All mitigation techniques improve on the statistical parity (first column). This is expected for the baseline approaches as they are specifically designed to remove average disparities between groups. 
We also note the difference in pre- and post-interview results. The increase in parity violation in Causal (Post) can be explained by the fact that it only adjusts for the outcome variable and assumes disparities in the interview score are acceptable. Disparities in score will in turn result in different outcomes across groups but in post-interview analysis this effect remains undetected. Finally, in terms of accuracy, Causal (Post) achieves comparable results to the other methods. The difference in the accuracy of Causal (Pre) and (Post) is in part due to the fact that the accuracy is measured with respect to the observed unfair outcomes. As a result, Causal (Pre) which significantly reduces the gap between female and male candidates may not conform to the historical decisions. Finally, these results highlight the importance of determining the timing of the intervention. Specifically,  
they suggest that through the causal framework, we are able to identify and remove sources of disparities by actively adjusting the affected variables. 
%is due to the fact that the former relies on one additional imputation step which introduces more error. 
Finally, we evaluated our approach based on causal criteria of fairness, choosing pre-interview as the starting time of fairness assessment. In Table~\ref{tab:res-total-causal}, we observe no violation of fairness in Causal (Pre) as expected. However, Causal (post) exhibits small violations which is due to the fact that it only mitigates unfairness due to $\gamma$ and in the hiring decision.
%, however, indicates that the model favors one group ($A=1$). This further suggests that in order 
%is due to the fact that in the former we adjust both the score values and outcome, whereas in the latter we only 
%We also consider the more challenging case of pre-interview unfairness mitigation as we need to impute counterfactual values of both the score $S(A)$ and outcome $Y(A)$. 
%summarizes the results. 
\begin{table}[t!]
    \centering
    \begin{tabular}{P{2.5cm}P{1.5cm}P{3cm}P{2cm}P{2cm}P{2cm}}
    \toprule
    \multirow{1}{*}{} & \multicolumn{4}{c}{Fairness Violation (Statistical Criteria)} & \\
    \cmidrule{2-5} & Parity & Positive Pred. Parity & E-Odds (TP) & E-Odds (FP) & Accuracy (\%) \\
    \hline
    No Fairness & 0.31 & 0.02 & 0.26 & 0.21 & 72.7 \\
    Re-weighting  & 0.10 & 0.11 & 0.04  & 0.03 & 71.8 \\
    PrejudiceRemover & 0.16 & 0.04 & 0.02 & 0.24 & 74.0 \\
    RejectOption & 0.05  & 0.19 & 0.09 & 0.16 & 72.0  \\
    Causal (Pre) & 0.03  & 0.14  & -0.02  & -0.04  & 70.0 \\
    Causal (Post) & 0.17 & 0.07 & -0.11 & -0.09 & 72.0\\
    \bottomrule
    \end{tabular}
\caption{Fairness violation of statistical criteria and the classification accuracy.}
\label{tab:res-total-stat}
\vspace*{-\baselineskip}
\end{table}


\begin{table}[h!]
    \centering
    \begin{tabular}{P{2.5cm}P{1.5cm}P{3cm}P{2cm}P{2cm}}
    \toprule
    \multirow{1}{*}{} & \multicolumn{4}{c}{Fairness Violation (Causal Criteria)} \\
    \cmidrule{2-5} & Parity & Positive Pred. Parity & E-Odds (TP) & E-Odds (FP) \\
    \hline
    Causal (Pre) & 0.00  & 0.00  & 0.00  & 0.00 \\
    Causal (Post) & 0.06 & 0.02 & 0.05 & 0.01 \\
    \bottomrule
    \end{tabular}
\caption{Fairness violation of causal criteria.}
\label{tab:res-total-causal}
\vspace*{-\baselineskip}
\end{table}

\newar
{
\subsection{Lending}

It is not within the scope of this paper to conduct empirical evaluation of discrimination in mortgage lending systems. As there is not enough information in the publicly available datasets. We draw samples from the US mortgage lending data set to contextualize our causal fairness framework. The Home Mortgage Disclosure Act (HMDA) requires collection and disclosure of individual-level data for lenders, including race and gender, which allows for greater transparency, accountability, and academic scrutiny in a domain with a history of contentious discriminatory practices. 


The lending process involves a series of activities that lead to the approval or rejection of a bank loan application.

Despite these limits on the internal validity of our analysis, this should not preclude the demonstration of methodologies. The following steps were taken to facilitate the analysis
}
\section{Conclusion}
As empirical evidence on ethical implications of algorithmic decision-making is growing~\cite{Rice2012DiscriminatoryColor,Monahan2016RiskSentencing,Obermeyer2019DissectingPeople,Simonite2020MeetCollege}, a variety of approaches have been proposed to evaluate and minimize the harms of these algorithms. In the statistical fairness literature, it is well-established that it is not possible to satisfy every fairness criterion simultaneously, which results in significant trade-offs in selecting a metric. 
On the other hand, in the causal fairness literature, there is substantial ambiguity around how the proposed methods should be applied to a particular problem. Also, these methods rely on assumptions that are often too strong to be applicable in practice. In this work, we addressed some of these limitations.

First, we illustrated the utility of applying concepts from the ``potential outcomes framework'' to algorithmic fairness problems. In particular, we emphasized the timing and nature of the intervention as two key aspects of causal fairness analysis. That is, for any valid causal analysis, it is critical to precisely define the starting point of the fairness evaluation and the postulated intervention. We argue that fairness evaluation is not a static problem and unfairness can happen at various points and within and across multiple domains. This is contrast with methods that rely on fixed DAG models. 

Next, we demonstrated how such a causal framework can address the limitations of existing approaches. Specifically, our theoretical investigation indicates that there is an inherent compatibility between the causal fairness definitions we propose. Finally, we showed the effectiveness of our approach in evaluating and mitigating unfairness associated with different stages of decision-making. We hope that our empirical observations spark additional work on collecting new datasets that lend themselves to temporal fairness evaluation. 

%\noindent\textbf{Mortgage Lending. }
%We also test our approach in the lending scenario using the real-world data from Home Mortgage Disclosure Act\footnote{The data is available at \url{https://ffiec.cfpb.gov/}.}. Each year thousands of financial institutions report data about mortgages to the public. The data helps show whether lenders are serving the housing needs of their communities and shed light on lending patterns that could be discriminatory. HMDA dataset has been used to investigate geography-based fairness~\cite{Chen2019FairnessUnobserved}. It consists of applicant's information such as income, loan amount, loan origination outcome as well as self-reported race/ethnicity. We will defer the details on the data pre-processing and preparation to the Appendix. We note that some information in the data is modified or missing (e.g., credit score) in order to protect borrower privacy. Nonetheless, we use this data to demonstrate how our approach can be used in practice. We denote $Y = 1$ if a loan application was approved or originated,
%and $Y = 0$ if it was denied. In the data, 68\% of the non-Hispanic whites and only 51\% of black applicants received a loan (there was not a significant difference between male and female borrowers).
%\noindent\textbf{Advertisement. }In advertising, algorithms are used to target for maximal impact and revenue, but recent studies found gender-based discrimination in who receives ads for STEM (science, technology, engineering, and mathematics) careers~\cite{Lambrecht2019AlgorithmicAds}. Motivated by the above examples, we collected a list of social domains along with the possible points of discrimination and we add to the list provided in~\cite{Quillian2006MeasuringDiscrimination}.   



==> new_material.tex <==
\section{Fair Evaluation Dataset}

When labels are subject to discrimination, current metrics do no provide a reliable evaluation of the machine learning models. However, this aspect is often ignored, i.e., validation datasets use for model evaluation are typically prone to different forms of bias. We can introduce a causal variant of common model evaluation metrics.  In particular, consider the 0-1 accuracy. In order to account for the potential unfairness in the labels, the accuracy of a model can be evaluated against the counterfactual values: $\E[\hat{Y} - Y(0)]$. 


==> related_work.tex <==
\section{Related Work}\label{sec:related}
%This paper is related to two streams of literature which we review. 
%\paragraph{Causal Inference}
There are two main frameworks for causal inference: structural causal models~\cite{Hitchcock2001Causality:Inference}, also referred to as DAGs, and the potential outcomes framework (POF)~\cite{Rubin2005CausalOutcomes}. DAGs can be viewed as a sequence of steps for generating a distribution from independent noise variables. Causal queries are performed by changing the value of a variable and propagating its effect through the DAG~\cite{Hitchcock2001Causality:Inference}. POF, on the other hand, starts by defining the counterfactuals with reference to an \emph{intervention} and postulates potential outcomes under different interventions, albeit some unobserved. In general, DAGs encode more assumptions about the relationships of the variables; i.e., one can derive potential outcomes from a DAG, but potential outcomes alone are not sufficient to construct the DAG. Consequently, POF has been more widely adopted in empirical research, including bias evaluation outside of ML~\cite{Bertrand2004AreDiscrimination,VanderWeele2014OnVariables}. More detailed discussion on the differences between the two frameworks in relation to empirical research can be found in~\cite{Imbens2020PotentialEconomics}. Causal inference on immutable attributes has appeared in several works including~\cite{VanderWeele2014OnVariables,Kilbertus2017AvoidingReasoning, gaebler2022causal}. \newar{Specifically, \citet{gaebler2022causal} also consider the timing of the perceiving one's sensitive attribute for determining the pre and post-treatment variables used in the causal effect analysis. However, their analysis is limited to estimating the level of discrimination and not mitigation.}


%via proxy variables and\newar{~\cite{Greiner2011CausalCharacteristics} through the perception of an immutable attribute. In this work, we follow the footsteps of~\cite{Greiner2011CausalCharacteristics} and  provide a rigorous framework to reason about the causal effect of immutable attributes which helps avoid some of the common issues in causal inference including post-treatment bias.}

Recently, there has been much interest in causality in the machine learning community, where the majority of works have adopted the DAG framework~\cite{Kusner2017CounterfactualFairness,Kilbertus2017AvoidingReasoning,Zhang2018FairnessFormula,Zhang2018EqualityApproach,Madras2019FairnessData,Chiappa2019PathspecificFairness} with a few exceptions that rely on POF~\cite{Nabi2018FairOutcomes,Khademi2019FairnessCausality}. Specifically,~\cite{Kusner2017CounterfactualFairness} provides an individual-based causal fairness definition that renders a decision fair towards an individual if it is the same in the actual world and a counterfactual world where the individual possessed a different sensitive attribute. In~\cite{Kilbertus2017AvoidingReasoning}, the authors propose \emph{proxy discrimination} as (indirect) discrimination via proxy variables such as name, visual features, and language which are more amenable to manipulation. Additionally,~\cite{Nabi2018FairOutcomes,Chiappa2019PathspecificFairness} study path-specific discrimination, where the former proposes to remove the descendants of the sensitive attribute under the unfair pathway and the latter aims to correct the those variables.~\citet{salimi2019interventional} also define causal fairness based on the notion of admissible variables, variables through which it
is permissible for the sensitive attribute to influence the outcome. They propose a data pre-processing approach to enforce it.~\citet{Khademi2019FairnessCausality} propose two causal definitions of group fairness: fair on average causal effect (FACE), and fair on average causal effect on the treated (FACT) and show how these quantities can be estimated for sensitive attributes as the treatment. The authors restrict their attention to the fairness evaluation task and do not discuss the distinction between pre- and post-treatment variables. Further,~\cite{Zhang2018FairnessFormula,Zhang2018EqualityApproach} discusses counterfactual direct, indirect, and spurious effects and provides formulas to identify these quantities from observational data. These works rely on a causal model, or DAG, and develop different methodologies to identify and mitigate unfairness. However, a clear discussion of the causal assumptions is typically missing, which consequently hinders the adoption of these methods in practice. In addition, the validity of the causal assumptions are influenced by the nature of the postulated intervention and its timing, which is not clearly articulated in the current literature. In many applications, discrimination by specific individuals or institutional actors is the subject of a study---not an entire causal pathway. Our work makes this distinction by highlighting the importance of specifying the timing of hypothetical intervention.
%Because race cannot be directly manipulated or randomly allocated to study participants, researchers must be able to translate ex- perimental results into a framework that allows them to address, in some form, causal statements regarding evidence of discrimination
%Works on causality go back 
%Most of such empirical works use PO framework as a formal basis for causal analysis. One explanation is that in general, DAGs encode more assumptions about the relationships of the variables, i.e., one can derive potential outcomes from a DAG, however, potential outcomes alone are not sufficient to construct the DAG. From a practical perspective, PO framework is more desirable. 
%In the empirical sciences, PO framework is frequently adopted to conduct causal analyses~\citet{Imbens2020PotentialEconomics}.
%These frameworks are complementary, with different strengths that make them particularly appropriate to address different questions~\cite{Imbens2020PotentialEconomics}. 
%In particular, DAGs provide an often clear and accessible way to visually express the key assumptions about the causal relationships between different variables. The PO framework starts by defining the potential outcomes with reference to an \emph{intervention} and views potential outcomes under different interventions as missing values. In econometrics literature, PO framework has witnessed great popularity, on the other hand, there is a lack of convincing empirical applications under the DAG framework~\citet{Imbens2020PotentialEconomics}. and has been widely adopted in recent years in the causal fairness literature. 
%By doing so, it makes a distinction between variables that are fixed pre-intervention and post-intervention also referred to as pre-treatment and post-treatment variables. In econometric literature, PO framework has witnessed great popularity. The reason, as articulated by~\citet{Imbens2020PotentialEconomics} is the lack of convincing empirical applications under the DAG framework. Similarly, most of the works on causal fairness has focused on DAG framework. However, one of most difficult parts which has hindered the adoption of these methods for bias mitigation is coming up with the right structural model. In fact, in many cases, arguing for the absence of a causal link between two variables is extremely difficult.
%\paragraph{Fairness in Machine Learning}

Finally, we briefly review the observational notions of fairness. Demographic parity and its variants have been studied in numerous papers~\cite{Dwork2012FairnessAwareness,Feldman2015CertifyingImpact,Corbett-Davies2017AlgorithmicFairness}. Also referred to as statistical parity, this fairness criteria requires the average outcome to be the same across different sensitive groups. Conditional statistical parity~\cite{Feldman2015CertifyingImpact,Corbett-Davies2017AlgorithmicFairness} imposes a similar requirement after conditioning on a set of legitimate factors. In the classification setting, equalized odds and a relaxed variant, equality of opportunity, have been proposed~\cite{Hardt2016EqualityLearning} to measure the disparities in the error rate across different sensitive groups. The aforementioned criteria can be expressed using probability statements involving the observed random variables at hand, hence the name observational. These criteria are often easy to state and interpret. \newar{However, they do not often appropriately account for relevant differences across individuals, e.g., coding experience in a software development job~\cite{dutta2021fairness}.} In addition, they suffer from a major limitation: it is impossible to simultaneously achieve these criteria on any particular dataset~\cite{Kleinberg2017InherentScores, Chouldechova2017FairInstruments,SolonBarocasMoritzHardt2020FairnessOpportunities}.
In this work, we revisit these notions and introduce their causal variants, where we show that under the causal framework, there is no fundamental disagreement between different criteria. \newar{For more detailed discussions, we refer the readers to the survey on fair machine learning~\cite{Mehrabi2021ALearning}.}
